Safe Data Collection for Offline and Online Policy Learning

Motivated by practical needs of experimentation and policy learning in online platforms, we study the problem of safe data collection. Specifically, our goal is to develop a logging policy that efficiently explores different actions to elicit information while achieving competitive reward with a baseline production policy. We first show that a common practice of mixing the production policy with randomized exploration, despite being safe, is sub-optimal in maximizing information gain. Then, we propose a safe optimal logging policy via a novel water-filling technique for the case when no side information about the actions' expected reward is available. We improve upon this design by considering side information and also extend our approaches to the linear contextual model to account for a large number of actions. Along the way, we analyze how our data logging policies impact errors in off(line)-policy learning and empirically validate the benefit of our design by conducting extensive numerical experiments with synthetic and MNIST datasets. To further demonstrate the generality of our approach, we also consider the safe online learning setting. By adaptively applying our techniques, we develop the Safe Phased-Elimination (SafePE) algorithm that can achieve optimal regret bound with only logarithmic number of policy updates.

==> Experiments.tex <==


\section{Experiments}
\label{sec:experiments}


We conduct three experiments. In \cref{sec:illustrative example}, we illustrate the basic properties of our approach on a simple example. We evaluate it on a diverse set of problems in \cref{sec:synthetic problems} and on the MNIST dataset in \cref{sec:mnist dataset}.

Our approach is implemented as described in \cref{sec:frank-wolfe} and we call it \safeod, which is an abbreviation for safe optimal design. We compare it with two baselines. The first baseline is the G-optimal design $\pi_g$. The G-optimal design can be viewed as an unsafe variant of \safeod, \ie, $\alpha=0$. The second baseline is a mixture policy $\pi_\mathrm{mix} = \alpha \pi_0 + (1 - \alpha) \mathbf{1}_K / K$. This policy is guaranteed to satisfy the safety constraint but may not maximize information gain.

All logging policies $\pi$ are evaluated by thee criteria:
\begin{itemize}
	\item The first is the \emph{design width} $\sqrt{g(\pi)}$, which is defined in \eqref{eq:g-optimal design} and reflects how well $\pi$ minimizes uncertainty over all actions. Lower values are better. 
	\item The second criterion is the \emph{safety violation} $\max_{\theta_* \in \Theta} (\alpha\pi_0 - \pi)\T A\T \theta_*$ (\cref{sec:general}), which measures how much $\pi$ violates the safety constraint for being close to the production policy $\pi_0$. Lower values are better. 
	\item The last metric is \emph{off-policy gap}, which measures the suboptimality of the best off-policy estimated action on data collected by $\pi$. This metric is computed as follows. First, we drawn $\theta_* \in \Theta$, uniformly at random, and find the best action $a_*$ under $\theta_*$. Second, we collect a dataset $\cD$ of size $n = 10 d$, were the noisy observation of action $a$ is $a\T \theta_* + \varepsilon$ for $\varepsilon \sim \cN(0, 1)$. Finally, we compute the MLE of $\theta_*$ from $\cD$, which we denote by $\hat{\theta}$, and find the best action $\hat{a}$ under $\hat{\theta}$. The off-policy gap is $(a_* - \hat{a})\T \theta_*$ and we estimate it from $1\,000$ random runs for any given logging policy, as described above.
\end{itemize} 


\subsection{Illustrative Example}
\label{sec:illustrative example}

In the first example, $\cA = \set{(1, 0), (0, 1)}$, $\pi_0 = (0.2, 0.8)$, and $\alpha = 0.9$; and $\Theta$ is given by $\bar{\theta} = (1, 2)$ and $\bar{\Sigma} = 0.1 I_2$. In this case, $\pi_0$ takes the most rewarding action with a high probability of $0.8$. Therefore, \safeod cannot be very different from $\pi_0$ and is ${\pie} = (0.330, 0.670)$. This design satisfies the safety constraint and its width is $1.74$. In comparison, the G-optimal design is $\pi_g = (0.5, 0.5)$ and obviously violates the safety constraint. For instance, even at $\bar{\theta}$, the constraint violation is $0.9 \cdot (0.2 \cdot 1 + 0.8 \cdot 2) - 0.5 \cdot 3 = 0.12$. However, its width is only $1.414$. The mixture policy $\pi_\mathrm{mix}$ satisfies the safety constraint but its width is $2.085$, about $15\%$ higher than in \safeod.

In the second example, we set $\bar{\theta} = (2, 1)$. In this case, $\pi_0$ takes the least rewarding action with a high probability of $0.8$. Therefore, \safeod can depart significantly from $\pi_0$ and is $\pie = (0.5, 0.5)$. This design satisfies the safety constraint and its width is $1.141$. The G-optimal design coincides with \safeod, \ie, $\pi_g = {\pie}$. The mixture policy $\pi_\mathrm{mix}$ also satisfies the safety constraint but its width is $2.085$.

In summary, \safeod combines the best properties of $\pi_g$ and $\pi_\textrm{mix}$. When the safety constraint is strict, \safeod satisfies it. When it is not, \safeod has a low width, similarly to the G-optimal design.


\subsection{Synthetic Problems}
\label{sec:synthetic problems}

We also experiment with the following randomly generated problems. The number of actions is $K = 100$ and their feature vectors are drawn uniformly from a $d$-dimensional unit sphere. The production policy $\pi_0$ is drawn uniformly from a $(K - 1)$-dimensional simplex. The set $\Theta$ is defined by $\bar{\Sigma} = I_d$ and $\bar{\theta}$, where the latter is drawn uniformly from a $d$-dimensional hypercube $[1, 2]^d$. We vary $d$ and $\alpha$, and have $50$ independent experiments for each setting.

In \cref{fig:d=4 alpha=0.900}, we report results for $d = 4$ and $\alpha = 0.9$. We observe that the G-optimal designs have low widths but also violate the safety constraint. On the other hand, the mixture policy always satisfies the safety constraint but leads to high design widths. \safeod strikes the balance between the two objectives, by minimizing the design width under the safety constraint. In all cases, design widths correlate with off-policy gaps.
\begin{figure}[!ht]
	\vspace{-0.1in}
	\centering
	\includegraphics[width=5.6in]{Figures/d=4_alpha=0900.pdf} \\
	\vspace{-0.2in}
	\caption{Comparison of \safeod to the G-optimal optimal design and the mixture policy, for $50$ random runs.}
	\label{fig:d=4 alpha=0.900}
\end{figure}

In \cref{fig:d}, we fix $\alpha = 0.9$ and vary $d$; while in \cref{fig:alpha}, we fix $d = 4$ and vary $\alpha$. In general, we observe that \safeod performs similarly to the G-optimal design whenever it is easy to satisfy the safety constraint, when the number of features $d$ is large or the safety parameter $\alpha$ is small. In all other cases, \safeod produces designs of higher widths and off-policy gaps in exchange for satisfying the safety constraint. The mixture policy always satisfies the safety constraint but leads to high design widths and off-policy gaps.
\begin{figure}[!ht]
	\vspace{-0.1in}
	\centering
	\includegraphics[width=5.6in]{Figures/d.pdf} \\
	\vspace{-0.2in}
	\caption{Comparison of \safeod to the G-optimal optimal design and the mixture policy. We fix the safety parameter at $\alpha = 0.9$ and vary $d$. Each safety violation is the fraction of violated safety constraints in $50$ runs.}
	\label{fig:d}
\end{figure}
\begin{figure}[!t]
	\vspace{-0.1in}
	\centering
	\includegraphics[width=5.6in]{Figures/alpha.pdf} \\
	\vspace{-0.25in}
	\caption{Comparison of \safeod to the G-optimal optimal design and the mixture policy. We fix $d = 4$ and vary the safety parameter $\alpha$. Each safety violation is the fraction of violated safety constraints in $50$ runs.}
	\label{fig:alpha}
\end{figure}
\subsection{MNIST Dataset}
\label{sec:mnist dataset}

The last experiment is conducted on the MNIST dataset \citep{lecun10mnist}. This experiment is a more realist variant of that in \cref{fig:d=4 alpha=0.900}, where the actions $\cA$ and the safety ellipsoid $\Theta$ are estimated from a real-world dataset.

\begin{figure*}[t]
	\centering
	\includegraphics[width=5.6in]{Figures/mnist_alpha=0900.pdf}
	\caption{Comparison of \safeod to the G-optimal optimal design and the mixture policy on the MNIST dataset.}
	\label{fig:mnist alpha=0.900}
\end{figure*}

This experiment is conducted as follows. First, we choose a random digit and assign it reward one. All remaining digits have reward zero. Second, we view the (flatten) feature vector of each digit as an action (see, \eg, \cite{Olah14}) and learn a least-squares regressor on these data. We set $\bar{\theta}$ and $\bar{\Sigma}$ to its weights and the inverse covariance matrix, respectively. These two quantities define $\Theta$, an ellipsoid that is likely to contain the optimal weights $\theta_*$. Finally, we choose feature vectors of $K = 100$ random digit images as the action set $\cA$. The production policy $\pi_0$ is drawn uniformly from a $(K - 1)$-dimensional simplex. This is repeated $50$ times and our results are reported in \cref{fig:mnist alpha=0.900}.

\begin{figure*}[!t]
	\centering
	\includegraphics[width=5.6in]{Figures/mnist_alpha.pdf}
	\caption{Comparison of \safeod to the G-optimal optimal design and the mixture policy on the MNIST dataset. We vary the safety parameter $\alpha$. Each safety violation is the fraction of violated safety constraints in $50$ runs.}
	\label{fig:mnist alpha}
\end{figure*}

We observe similar trends to \cref{fig:d=4 alpha=0.900}. The G-optimal designs have a bit lower widths and better off-policy performance than \safeod, but can significantly violate the safety constraint. The comparable widths and off-policy performance of \safeod indicate that the cost of satisfying the safety constraint in real-world data may be low. The mixture policy always satisfies the safety constraint but leads to the highest design widths and worst off-policy performance.



As in \cref{fig:alpha}, we vary $\alpha$ in \cref{fig:mnist alpha}. For all $\alpha$, \safeod performs similarly to the G-optimal design but never violates the safety constraint. Again, the mixture policy always satisfies the safety constraint but leads to high design widths and off-policy gaps. This experiment shows that all observed trends in \cref{fig:mnist alpha=0.900} generalize beyond $\alpha = 0.9$.

